Locality-Aware Hyperspectral Classification

Hyperspectral image classification is gaining popularity for high-precision vision tasks in remote sensing, thanks to their ability to capture visual information available in a wide continuum of spectra. Researchers have been working on automating Hyperspectral image classification, with recent efforts leveraging Vision-Transformers. However, most research models only spectra information and lacks attention to the locality (i.e., neighboring pixels), which may be not sufficiently discriminative, resulting in performance limitations. To address this, we present three contributions: i) We introduce the Hyperspectral Locality-aware Image TransformEr (HyLITE), a vision transformer that models both local and spectral information, ii) A novel regularization function that promotes the integration of local-to-global information, and iii) Our proposed approach outperforms competing baselines by a significant margin, achieving up to 10% gains in accuracy. The trained models and the code are available at HyLITE.

==> 3-method-v0.tex <==




%\section{Locality-Aware ViT for Hyperspectral Sensing}
\section{Locality-aware Hyperspectral Image Transformer}

\partitle{Overview.} The overall framework of the proposed method is shown in Figure \ref{fig:architecture}, which is adopted from the SpectralFormer~\citep{hong2021spectralformer}. The network consists of three main parts, a linear projection layer, a transformer encoder module, and a multi-layer perceptron (MLP) head. The linear projection layer is used to project the flattened spatial patches to tokens with a desired length. The MLP head consists of one fully-connected layer to project the global $class$ embedding to class predictions. The transformer encoder includes several transformer blocks and cross-layer fusion (CAF) modules. The CAF modules are used to replace the skip connections in ViT by Hong et al.~\citep{hong2021spectralformer} by fusing the representations of the $l_{th}$ layer with the $(l-2)_{th}$ layer. According to ~\citep{hong2021spectralformer}, CAF gains better information exchange between layers and less information loss than using skip connection for HISC, which is also proved in our experiments. Thus, we keep the same setup of CAF as~\citep{hong2021spectralformer} in the proposed network. Different from the SpectralFormer, a spatial multi-head attention module is added between the spectral multi-head attention module and the feed-forward module in each transformer block. For the studied datasets, same as the SpectralFormer, we built 5 blocks and each attention module has 4 heads. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.86\textwidth]{figures/architecture.pdf}
    \caption{Overall framework of the proposed approach. First, given a hyperspectral patch, we patchify the input. Patchified input is then linearly projected, and processed by our model. Our model consists of several blocks of multi-head attention, which combines spatial and spectral attention. To further increase the information retention across layers, we also use cross-layer adaptive fusion (CAF). }
    \label{fig:architecture}
\end{figure}

\partitle{Spectral-Spatial Attention.}
The spectral-spatial attention mechanism combines both spectral attention and spatial attention in each transformer block. The spectral attention aims to model the spectral dependencies among the embedded spatial tokens, while the spatial attention is to capture the similarities of the entire spectral bands among each pixel. In detail, in the spectral attention module, we first calculate query, key, and value tensors from $\boldsymbol{Q}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_Q\right) \in \mathbb{R}^{(m+1) \times d}$, $\boldsymbol{K}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_K\right) \in \mathbb{R}^{(m+1) \times d}$, and $\boldsymbol{V}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_V\right) \in \mathbb{R}^{(m+1) \times d}$.
% $$\begin{aligned} & \boldsymbol{Q}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_Q\right) \in \mathbb{R}^{B \times P^2} \\ & \boldsymbol{K}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_K\right) \in \mathbb{R}^{B \times P^2} \\ & \boldsymbol{V}=\mathcal{F}\left(\boldsymbol{X} ; \boldsymbol{W}_V\right) \in \mathbb{R}^{B \times P^2} \\ & \end{aligned}$$
In which, $\boldsymbol{W}_Q$, $\boldsymbol{W}_K$, and $\boldsymbol{W}_V$ represent trainable parameters in the linear operation $\mathcal{F}$ of query, key, and values tensors, respectively. $X$ denotes the input tensor and $m$ represents the length of spectral bands. As a result, the spectral attention map is calculated as follows:
$$
\operatorname{spectral\_attn}=\operatorname{Softmax}\left(\frac{ \boldsymbol{Q} \cdot \boldsymbol{K}^T }{\sqrt{s} }\right) \in \mathbb{R}^{(m+1) \times (m+1)}
$$
in which $s$ denotes the scale factor. Then, the output of the spectral attention module is produced with:
$$
\operatorname{spectral\_out}= {spectral\_attn} \cdot V =\operatorname{Softmax}\left(\frac{ \boldsymbol{Q} \cdot \boldsymbol{K}^T }{\sqrt{s} }\right) \cdot V \in \mathbb{R}^{(m+1) \times d}
$$
In order to perform spatial attention, the output of the spectral attention module is permuted to $X^\prime \in \mathbb{R}^{d \times (m+1)}$. Similarly, the spatial attention is calculated as follows:
$$
\operatorname{spatial\_attn}=\operatorname{Softmax}\left(\frac{ \boldsymbol{Q^\prime} \cdot \boldsymbol{K^\prime}^T }{\sqrt{s} }\right) \in \mathbb{R}^{d \times d}
$$
in which $\boldsymbol{Q^\prime}=\mathcal{F}\left(\boldsymbol{X^\prime} ; \boldsymbol{W}_{Q^\prime}\right) \in \mathbb{R}^{d \times (m+1)}$, and $\boldsymbol{K^\prime}=\mathcal{F}\left(\boldsymbol{X^\prime} ; \boldsymbol{W}_{K^\prime}\right) \in \mathbb{R}^{d \times (m+1)}$. The output of the spatial attention module is calculated with:
$$
\operatorname{spatial\_out}= {spatial\_attn} \cdot V^{\prime} =\operatorname{Softmax}\left(\frac{ \boldsymbol{Q^\prime} \cdot \boldsymbol{K^\prime}^T }{\sqrt{s} }\right) \in \mathbb{R}^{d \times (m+1)}
$$
Finally, the output of the spatial attention module is permuted back to the original shape of $X \in \mathbb{R}^{(m+1) \times d}$, and then passed to the feed forward module.
% Following previous works~\citep{khan2022transformers, hong2021spectralformer}, 
\partitle{Global-Local Alignment Loss.} Inspired by the performance gain of global-local feature alignment technique for masked unsupervised learning tasks~\citep{limasked}, we add extra global-local feature alignment loss in addition to cross-entropy loss. Following the work of Li et al.~\citep{limasked}, the global-local feature alignment loss is defined as the average squared distance between the global $class$ token and all $patch$ tokens: $\mathcal{L}_{\text {align }}=\frac{1}{N m} \sum_{n=1}^N \sum_{i=1}^m\left\|v_n^c-v_n^i\right\|_2^2$, in which $N$ is the batch size, $m$ denotes the number of spectral bands which is also the number of embedded patch tokens, $v_n^c$ represents the embedded global $class$ token, and $v_n^i$ denotes $i\_th$ $patch$ token embedding. This alignment loss aims to aggregate local $patch$ features into global $class$ feature for better classification performance. Hence, the overall loss of the proposed method is defined as $\mathcal{L} = \mathcal{L}_{\text {cross\_entropy }} + \lambda_{align}\mathcal{L}_{\text {align }}$, in which $\lambda_{align}$ denotes the weight of the alignment loss and has a value of $[0,1]$. $\lambda_{align}=1$ was set in out experiments as it works the best among all studied values.

\partitle{ViT Architecture.} In details of the workflow of the proposed architecture, given an input hyperspectral image with a size of $m \times H \times W$ where $m$ represents the number of spectra channels and $H \times W$ stands for the spatial size of the entire image, it is firstly split into a number of overlapping spatial patches with a shape of $m \times p \times p$ where $p$ is the specified patch size. After patchifying, each patch is unfolded along the spatial dimension to a 2-D vector with a shape of $m \times p^2$, and then is input as a sequence of spatial vectors along the spectral dimension to the linear projection layer. The sequence of each patch has a length of $m$. The linear projection layer projects the flattened spatial patches into embedded tokens with a desired length. In addition, to capture positional information among tokens, a randomly initialized learnable positional embedding is added to each token. Meanwhile, a global $class$ token is also added to learn the global feature representation. After adding the global $class$ token and the positional encoding, the input sequence with a shape of $(m+1, p^2)$ is passed to the transformer encoder. With the proposed transformer blocks, the spectral dependencies of each spatial token is captured via the multi-head spectral attention modules, and then the similarity of the entire spectral bands between each pixel inside the same patch is extracted from the spatial attention modules. Therefore, features are extracted globally and locally from the transformer encoder and fed into the MLP head for the final classification.


 \mert{Fit on two pages including implementation details.}

==> 3-method-v1.tex <==


\vspace{-5mm}

%\section{Locality-Aware \hyper{} Image Transformer}
\section{Hyperspectral Locality-Aware Image TransformEr}
\label{sec:method}
%%%% Plan for the method %%%%

% First, give an overview of the input signal. 
% Then, give an overview of the whole flow within the network
% Then, talk about: 1) Local-Spectral Attention, 2) Local-Spectral Regularization, 3) Architecture (\ie CAF etc.)

% While giving Local-Spectral Attention, it is good to give an overview of QKV attention and then specialize it for local and spectral. Also emphasize the importance of order. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/architecture_v2.pdf}
    %\caption{Overall framework of the proposed approach. First, given a \hyper{} patch, we patchify the input. Patchified input is then linearly projected, and processed by our model. Our model consists of several blocks of multi-head attention, which combines spatial and spectral attention. To further increase the information retention across layers, we also use cross-layer adaptive fusion (CAF). \mert{Fangqin: please include regularization loss.} }
    %\caption{An overview of system. system takes a \hyper{} image as input, and then classifies each pixel. To perform this, we first patchify the input cube to $p\times p$ sized patches. Then, we apply linear projection on top of the patches, and process them via multiple, multi-head self-attention blocks (MHA). Within each block, we alternate between spectral and local attention followed by a feed-forward layer. Finally, we aggregate the information across layers via Cross-Adaptive Fusion (CAF), and compute the loss function to update the transformer weights. \mert{Think about how to simplify this graph and caption. currently crowded.}}
    %\caption{An overview of system. system is a vision transformer for \hyper{} image classification. system achieves categorization in four steps: i) Preprocessing via patchifying and linear-projecting the input, ii) Attending on local-spectral information, iii) Classification and iv) Regularization. Please see the text for the details. \mert{Think about how to declutter this Figure.}}
%    \caption{An overview of \system{}. \system{} achieves \hyper{} classification in four steps: \textit{i)} \textcolor{magenta}{Preprocessing} the input by patchifying the image, \textit{ii)} \textcolor{cyan}{Representing} local-spectral visual variation using Transformer encoder, which consists of multiple blocks of spectral and local multi-head attention (MHA), \textit{iii)} \textcolor{amber}{Classifying} the input, finally \textit{iv)} \textcolor{orange}{Regularizing} local-spectral representations. Best viewed in color.}
\caption{An overview of \system{}. \textcolor{magenta}{\textit{i). Preprocessing}}: The input image is patchified, linearly projected, and appended with a classifier token and positional information. \textcolor{cyan}{\textit{ii). Representation}}: Input is further processed by identical blocks of spectral and local multi-head attention (MHA) blocks. \textcolor{amber}{\textit{iii). Classification}}: At the end, the representation of the classifier token is assigned to a distinct category, such as $\{grass, road\}$. \textcolor{orange}{\textit{iv). Regularization}}: To further promote locality, we apply our novel regularization on top of the learned token representations.}
    \label{fig:architecture}
\end{figure}



An overview of \system{} is given in Figure~\ref{fig:architecture}. We are given a tuple of \hyper{} image-label pair, $(I, y)$ where $I \in\Ree^{m\times w\times h}$ and $y \in\Ree^{w\times h}$. Here, $m$ is the spectral resolution, and $w\times h$ is the spatial resolution (width-height), respectively. Pixels are labeled with a mutually exclusive category, such as $\{grass, road\}$. We map the input image into pixel-wise predictions via $I\xrightarrow{g_{\theta}(\cdot)}y^{\prime}$, where $g_{\theta}(\cdot)$ is a vision-transformer with parameters $\theta$. 

Following the protocol in~\citep{hong2021spectralformer}, the input image is divided into  $N$ square patches: $I \in \Ree^{N\times (m\times p^2)}$, with patch-size $p$ (\ie $7\times 7$). $N$ is equal to the total number of pixels $N=w\times h$ as the patches are overlapping. Each patch is a distinct training instance, and the goal is to predict the category of the center pixel. 

Let's denote with $x$ each such signal where $x \in\Ree^{m\times p^2}$. Here, the signal consists of $m$ spectral tokens, each with $p^2$ number of pixels $x = [z^{1}; z^{2}; ...; z^{m}]$ where $z^{i} \in\Ree^{1\times p^2}$. Then, \system{} consists of four main steps, namely preprocessing, representation, classification, and finally regularization: 

\partitle{1) \textul{Preprocessing}.} First, the input is appended with a learnable class token $z^{0} \in\Ree^{1\times d}$. And then, we apply linear projection $W\in\Ree^{p^2\times d}$ and add a learnable position information tensor $P \in\Ree^{(m+1)\times d}$. Formally, the input tensor takes the form: %$x_{0} = [z^{0}; z^{1}W; z^{2}W; ...; z^{m}W] + P \in \Ree^{(m+1)\times d}$. 
\begin{align}
\label{equ:prep}
 x_{0} &= [z^{0}; z^{1}W; z^{2}W; ...; z^{m}W] + P \in \Ree^{(m+1)\times d} 
\end{align}

%%%%%%%%%%%% V2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\partitle{2) \textul{Representation}.} The preprocessed input is then further processed by $B$ blocks of representation layers, which is a stack of Spectral-Attention Layer ($S$), Local-Attention Layer ($L$) and Feed-Forward Layer ($F$). Here, the order of spectral and local attention matters, which will be shown via experiments. Before each sub-layer, a LayerNorm~\citep{ba2016layer} operation is performed, which we omit for clarity. Formally, all $B$ blocks operate as: %$x_{b} = FF(L(S(x_{b-1}))),  \in \Ree^{(m+1)\times d}, b=1\ldots B$.
\begin{align}
  x_{b} &= F(L(S(x_{b-1}))),  \in \Ree^{(m+1)\times d}  & b=1\ldots B  
\end{align}

\noindent Both the local-attention and the spectral-attention layers are implemented via self-attention. A self-attention layer takes three different projections of the same input, namely query, key and value, and then calculates a weighted average of the input by highlighting distinctive features. 

Self-attention is computed with $x = self(q,k,v) = softmax(\frac{qk^{T}}{\sqrt{d}})v$. Here, $[q, k, v]$ are the linear-projections $[q, k, v] = [xW_{q}, xW_{k}, xW_{v}]$  of the input feature $x$, and $W_{self} = \{W_{q}, W_{k}, W_{v}\}$ are the parameters of the projection. 

%Our representation block alternates between spectral-attention $S(\cdot)$, local-attention $L(\cdot)$ and feed-forward $FF(\cdot)$ layers. 

In spectral-attention, the emphasis is on the spectral dimension, hence the set of projections are parameterized by: $W_{self}^{s} = \{W_{q}^{s}, W_{k}^{s}, W_{v}^{s}\}$ with identical tensor dimensions of $\Ree^{(m+1)\times (m+1)}$. 

In local-attention, the emphasis is on the local dimension, hence the projections are parameterized by $W_{self}^{l} = \{W_{q}^{l}, W_{k}^{l}, W_{v}^{l}\}$ with identical tensor dimensions of $\Ree^{d\times d}$. 

Finally, the feed-forward layer $F(\cdot)$ is a one-layer MLP that computes the output of the block, which will be used to classify and regularize the representations. 

\partitle{3) \textul{Classification}.} Using the output of the classifier token, we project the local-spectral representation to the prediction space using a linear classifier $C\in\Ree^{d\times c}$ as: %$y^{\prime} = C(x_{B}^{0})  \in \Ree^{1\times c}$. 
\begin{align}
    y^{\prime} &= (x_{B}^{0} \cdot C)  \in \Ree^{1\times c}
\end{align}
\noindent where $x_{B}^{0} \in\Ree^{1\times d}$ is the classifier token representation (\ie $z^{0}$) from the last block $B$. 

\partitle{4) \textul{Regularization}.} Finally, using the classifier and spectral-token representations, we compute our novel regularization loss function on top of the last layer activations. Our model is trained by minimizing the following objective:  %$Reg(x_{B}^{0}, x_{B}^{i>0})$ which are detailed in the following Section.
\begin{align}
    \mathcal{O} = CE(y, y^{\prime}) + \lambda \cdot Reg(x_{B}^{0}, x_{B}^{i>0})
    \label{eq:loss}
\end{align}
\noindent where $CE(\cdot)$ is the standard cross-entropy, $Reg(\cdot)$ is our proposed local-spectral regularization loss, and $\lambda$ is the magnitude of the regularization which is simply set to $1$, and we refer the reader to our supplementary for results with different values. 

\hyper{} classification is different from traditional image classification, in the sense that spatial input resolution is quite small (\ie $7\times 7$) whereas spectral resolution is large (\ie $200$). To that end, when training a vision-transformer, we observe the following phenomenon: The global classifier token attends to only a few spectra, neglecting the local context. In the meanwhile, spectral tokens mostly attend to their self-representation, neglecting  the global context. To enforce aggregation of local-global context, we propose the following simple objective: 
\begin{align}
    \text{Reg} = \frac{1}{m}\sum_{i=1}^m\left\| x_{B}^{0} - x_{B}^{i} \right\|
\end{align}

%%%% V1 %%%%%%
%\noindent where we simultaneously enforce: \textit{i)} Global token $x_{B}^{0}$ to be as similar as possible to the average of local spectral representations. This leads to global token pooling information from \textit{all} local spectral bands, effectively incorporating local context. \textit{ii)} Local spectral token representation $x_{B}^{i>0}$ to be as similar as possible to the global token representation. This forces the local token to pool information from many other local spectral bands, effectively incorporating global context. As we will show, such a term has a significant effect on classification performance. 


%%%% V2 %%%%% 
\noindent To satisfy this loss function, first, the global token $x_{B}^{0}$ has to be similar to all the other spectral tokens $x_{B}^{i>0}$. This enforces the global token to aggregate information from multiple spectra, hence incorporating the spectral locality. Simultaneously, the spectral tokens have to be similar to the global token. This enforces the spectral tokens to aggregate information from the \textit{other} spectral tokens, hence incorporating the global context. As we will show, such a term has a significant effect on classification performance.

%$\mathcal{O} = CE(y, y^{\prime}) + \lambda \cdot Reg(x_{B})$
%\begin{align}
%    \mathcal{O} &= CE(y, y^{\prime}) + \lambda \cdot Reg(x_{B})
%\end{align}

%\noindent 


%\begin{itemize}[leftmargin=*]
%    \item \textit{Preprocessing:} First, the input is appended with a learnable class token $z^{0} \in\Ree^{1\times d}$. And then, we apply linear projection $W\in\Ree^{p^2\times d}$ and add a learnable position information tensor $P \in\Ree^{(m+1)\times d}$. 
%    \item \textit{Attention}: Preprocessed input is then further processed by $L$ blocks of local-spectral attention layers, which is a stack of Spectral-Attention Layer ($S$), Local-Attention Layer ($L$) and Feed-Forward Layer ($FF$). Here, the order of spectral and local attention matters, which will be shown via experiments. Before each sub-layer, a LayerNorm operation is performed, which we omit for clarity. 
 %   \item \textit{Fusion}: To preserve the information across all layers, following~\citep{hong2021spectralformer}, we apply Cross-Adaptive Fusion (CAF) between the output of the previous $(l-2)$-th layer and the input of the current $(l)$-th layer. The representations of these two layers are fused with a $1 \times 2 $ convolution layer. We refer to Hong et al.~\citep{hong2021spectralformer} for more details.
 %   \item \textit{Classification}: Finally, using the output of the classifier token, we project the local-spectral representation to the prediction space using a linear classifier $C\in\Ree^{d\times c}$. 
%\end{itemize}
%\subsection{Local-Spectral Representation and Regularization}
%\label{sec:components}
%Here, we detail our local-spectral representation and local-spectral regularization. 

%\partitle{Representation.} Both the local and the spectral attentional layers are implemented via self-attention. A self-attention layer takes as input three different projections of the same input, namely query, key and value, and then calculates a weighted average of the input by highlighting distinctive features. 

%Self-attention is computed with $x = self(q,k,v) = softmax(\frac{qk^{T}}{\sqrt{d}})v$. Here, $[q, k, v]$ are the linear-projections $[q, k, v] = [xW_{q}, xW_{k}, xW_{v}]$  of the input feature $x$, and $W_{self} = \{W_{q}, W_{k}, W_{v}\}$ are the parameters of the projection. 

%Our representation block alternates between spectral-attention $S(\cdot)$, local-attention $L(\cdot)$ and feed-forward $FF(\cdot)$ layers. In spectral-attention, the emphasis is on the spectral dimension, hence the set of projections are parameterized by: $W_{self}^{s} = \{W_{q}^{s}, W_{k}^{s}, W_{v}^{s}\}$ with identical tensor dimensions of $\Ree^{(m+1)\times (m+1)}$. In local-attention, the emphasis is on the local dimension, hence the projections are parameterized by $W_{self}^{l} = \{W_{q}^{l}, W_{k}^{l}, W_{v}^{l}\}$ with identical tensor dimensions of $\Ree^{d\times d}$. Finally, the feed-forward layer is a single-layer MLP that generates the output tensor of the block. 

%A self-attention layer computes three different representations, namely query, key, and value via $[q, k, v] = [xW_{q}, xW_{k}, xW_{v}]$, where $\{W_{q}, W_{k}, W_{v}\}$ are all linear-projections of the input. Then, the output of the layer is simply computed as: $x = softmax(\frac{qk^{T}}{\sqrt{d}})v$

%\begin{align}
% x = softmax(\frac{qk^{T}}{\sqrt{d}})v
%\end{align}

%\noindent In Spectral-Attention, the goal is to model the relationship across the spectrum, so linear projections are parameterized as: $\{W_{q}^{s}, W_{k}^{s}, W_{v}^{s}\}$ all with the dimensionality of $\Ree^{m\times m}$. 

%Similarly, in Local-Attention, the goal is to model the relationship across spatial pixels, to that end, linear projections are parameterized as: $\{W_{q}^{l}, W_{k}^{l}, W_{v}^{l}\}$ all with the dimensionality of $\Ree^{d\times d}$. The output of the spectral attention layer is fed through the local-attention, which is then finally projected by feed-forward layer before passing through another block. 

%\partitle{Regularization.} Our model is trained by minimizing the following objective: 
%\begin{align}
%    \mathcal{O} = CE(y, y^{\prime}) + \lambda \cdot Reg(x_{B}^{0}, x_{B}^{i>0})
%    \label{eq:loss}
%\end{align}
%\noindent where $CE(\cdot)$ is the standard cross-entropy, $Reg(\cdot)$ is our proposed local-spectral regularization loss, and $\lambda$ is the magnitude of the regularization which is simply set to $1$, and we refer the reader to our supplementary for results with different values. 

%\hyper{} classification is different from traditional image classification, in the sense that spatial input resolution is quite small (\ie $7\times 7$) whereas spectral resolution is large (\ie $200$). To that end, when training a vision-transformer, we observe the following phenomenon: The global classifier token attends to only few pixels, neglecting the local context. In the meanwhile, local pixels mostly attend to their self-representation, neglecting  the global context. To enforce accurate representation of local-global context, we propose the following simple objective: 
%\begin{align}
%    \text{Reg} = \frac{1}{m}\sum_{i=1}^m\left\| x_{B}^{0} - x_{B}^{i} \right\|
%\end{align}
%\noindent where we simultaneously enforce: \textit{i)} Global token $x_{B}^{0}$ to be as similar as possible to the average of local representations. This leads to a global token to pool information from \textit{all} local pixels, effectively incorporating global context. \textit{ii)} Local token representation $x_{B}^{i>0}$ to be as similar as possible to the global token representation. This forces the local token to pool information from many other local pixels, effectively incorporating local context. As we will show, such term has a significant effect on the classification performance. 

%effectively mitigating the aforementioned issues, yielding significant gain over the compared baselines. 

%This leads to the following: \textit{i).} The classifier token selects and attends to only a few pixels within the input, effectively losing the global context. \textit{ii).} On the other hand, local-spectral tokens mostly attend on their own representation (\ie self-only), effectively losing the local context. To simultaneously circumvent this, we propose the following objective function: $ \text{Reg} = \frac{1}{m}\sum_{i=1}^m\left\| x_{L}^{0} - x_{L}^{i} \right\|$. 

%This expression forces the classifier context to be close to the average of all the local pixels while forcing all local pixel representations to be close to the global classifier context, effectively circumventing the aforementioned issue. 

%As we will show, such regularization leads to a drastic improvement in performance, thanks to its ability to retain and represent locally global contextual features. 



%%%%%%%%%%%%%%%%%%%%%%%%%%% V2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\partitle{Overview.} An overview of \system{} is given in Figure~\ref{fig:architecture}. We are given a tuple of \hyper{} image-label pair $(I, y)$ each with size $\Ree^{m\times w\times h}$. Here, $m$ is the number of spectral bands, and $w\times h$ is the width-height of the image. The goal is to learn the mapping: $I\xrightarrow{g_{\theta}(\cdot)}y^{\prime}$, where $g_{\theta}(\cdot)$ is a vision-transformer parameterized by $\theta$, $y^{\prime}$ is the pixel-wise predictions, such as road, building, tree, etc. We drop $\theta$ from now on for clarity. We optimize $g(\cdot)$ via minimizing the following objective: 

%An overview of \system{} is presented in Figure~\ref{fig:architecture}. \system{} takes as input a \hyper{} image cube, and then classifies each pixel within the cube into their corresponding category, such as $\{road, building, tree\}$. 

%In \hyper{} image classification, we are given an input image cube $I \in\Ree^{m\times w\times h}$, where $m$ is the number of spectral bands, typically around hundreds, and $w$ is the width of the cube and $h$ is the height of the cube. Then, our goal is to train a deep neural network $g(\cdot)$, to map the input cube to per-pixel predictions, such as $\{road, building, tree\}$. 

%Formally, we are given input tuples $(I, y)$ as input, where  $I \in\Ree^{m\times w\times h}$ is the input image with $m$ spectral bands, $w\times h$ corresponds to width and height, and $y$ is the per-pixel class-labels the same size as the input. Our goal is to train a neural network $g_{\theta}(\cdot)$ with parameters $\theta$ to map the input image to class predictions as $I\xrightarrow{g_{\theta}(\cdot)}y^{\prime}$, where $y^{\prime}$ denotes the predictions. In this paper, the neural network $g_{\theta}(\cdot)$ is a Vision-Transformer, and we optimize the weights via minimizing the following objective: 

%\begin{align}
%\label{equ:main}
%\mathcal{L} = CE(g(I), y) + \lambda \cdot Reg(\cdot)
%\end{align}

%\noindent Here, $CE(\cdot)$ corresponds to standard cross-entropy loss, $Reg(\cdot)$ is our novel spatio-spectral regularization term, and $\lambda$ balances the contribution of the two losses. 

%To achieve this, we first split the input image into N, non-overlapping patches of $p\times p$, such that the input signal becomes: $I = [x_{1}, x_{2}, ..., x_{N}]$ where $x_{i} \in \Ree^{m\times p^{2}}$. 

%All the input then goes through a linear projection layer from the spatial dimension: $\Ree^{m\times p^{2}}\rightarrow\Ree^{m\times d}$. 

%Then, we append a classifier token $z_{0} \in \Ree^{1\times d}$ as $x_{i} = [z_{0}, z_{1}, ..., z{t}]$  to collect the features to perform the final classification for each patch. 

%We combine each input with positional embeddings to preserve location information. 

%Now, the input signal is ready to be processed by spectral and local attention layer blocks, which we describe below. 


%\subsection{Local-Spectral Multi-Head Self-Attention Block}

%Our model consists of multiple blocks of local and spectral attentional block, see Figure~\ref{fig:architecture}. A block mainly consists of three sub-layers: $x^{\prime}_{i} = FF(L(S(x_{i})))$, where $S(\cdot)$ corresponds to spectral attention layer, $L(\cdot)$ corresponds to local attention layer followed by $FF(\cdot)$ feed-forward projection layer. The input to each layer is normalized by LayerNorm~\citep{xxx} as is the best practice in vision-transformers. Below, we detail spectral and local attention. 

%\partitle{Spectral Multi-Head Attention.} In Spectral MHA, the goal is to model the relationship across different spectrum. To achieve this, we use multiple heads of self-attention layers~\citep{xxx}. A self-attention layer consists of three sub-networks, namely query, key and value networks, parameterized by $\{W_{Q}^{S}, W_{K}^{S}, W_{V}^{S}\}$ respectively, all with the dimensions $\Ree^{(m+1)\times (m+1)}$. Then, the output of spectral attention is calculated as: 


%\begin{align}
%    softmax(\frac{\mathcal{Q^{S}}\cdot\mathcal{K^{S^{\prime}}}}{\sqrt{d}})\cdot V^{S} \in \Ree^{(m+1)\times d}
%\end{align}

%\noindent where $\mathcal{Q^{S}}, \mathcal{K^{S}}, \mathcal{V^{S}}  =  W_{Q}^{S}x_{i}, W_{K}^{S}x_{i}, W_{V}^{S}x_{i}$ respectively. This allows the model to build sufficient representation to be further processed by the local attention, which we describe below. 

%\partitle{Local Multi-Head Attention.} In Local MHA, the goal is to model the relationship across different spectrum. To achieve this, we use multiple heads of self-attention layers~\citep{xxx}. A self-attention layer consists of three sub-networks, namely query, key and value networks, parameterized by $\{W_{Q}^{L}, W_{K}^{L}, W_{V}^{L}\}$ respectively, all with the dimensions $\Ree^{d\times d}$. Then, the output of spectral attention is calculated as: 

%\begin{align}
%    softmax(\frac{\mathcal{Q^{L^{\prime}}}\cdot\mathcal{K^{L}}}{\sqrt{d}})\cdot V^{L^{\prime}} \in \Ree^{d\times (m+1)}
%\end{align}


%\noindent where $\mathcal{Q^{L}}, \mathcal{K^{L}}, \mathcal{V^{L}}  =  W_{Q}^{L}x_{i}, W_{K}^{L}x_{i}, W_{V}^{L}x_{i}$ respectively.

%\begin{align}
%    [\mbf{q}, \mbf{k}, \mbf{v}] &= \mbf{z} \mbf{U}_{qkv}
%    & \mbf{U}_{qkv} &\in \mathbb{R}^{D \times 3 D_h} , \label{eq:qkv} \\
%    A &= \op{softmax}\left(\mbf{q}\mbf{k}^\top / \sqrt{D_h}\right)
%    & A &\in \mathbb{R}^{N \times N} , \label{eq:attn_matrix}\\
%    \op{SA}(\mbf{z}) &= A\mbf{v}\,. \label{eq:selfattn}
%\end{align}

%\begin{align}
%    [Q, K, V] = [W_{Q}z, W_{K}z]  
%\end{align}



%\partitle{Local-Spectral Regularization.}

%\partitle{Local-to-Spectral Attention.}

%\mert{L means many things. Fix this inconsistency!}


==> 4-2-experiments-v0.tex <==





\section{Hyperspectral Image Classification}

\subsection{Comparison to State-of-the-Art}

% Candidates: 
% vanilla comparison
% compressed comparison
% transfer learning: indian to houston, indian to pavia
% low-shot learning

The first experiment is to compare the proposed method to SoTA, namely ViT based SpectralFormer and Masked Auto-encoder based MAEST model. The results are shown in Table \ref{tab:sota1}, in which the best classification scores are displayed in bold together with its performance gains in comparison to SpectralFormer. 

\input{figures/table_sota}

Be aware that except for MAEST and SpectralFormer, the results of other baslines listed in Table \ref{tab:sota1} are taken from ~\citep{hong2021spectralformer} since our approach is built based on the SpectralFormer. It is clear that our model beats both SpectralFormer and MAEST on all three studied datasets without any pre-training. Particularly, our method gained $10.83\%$ and $6.64\%$ test OA comparing to SpectralFormer with Indian Pipes and Pavia University dataset respectively. 
% It is also worth noting that our intermediate model with only adding global-local alignment loss on top of SpectralFormer improves classification performance in a certain level. This proves that final classification benefits from aggregating local patch information. 

In addition, we have also compared our final model to SpectralFormer on varied size of sub-training samples of Indian Pines dataset. The subsets were randomly selected from the given training set listed in Table \ref{tab:IP}. As shown in Figure \ref{fig:ip_sub}, our method outperforms SpectralFormer for all the subsample sizes. Notably, our model reached over $80\%$ test OA with only $40\%$ of the training samples, which works even slightly better than SpectralFormer trained on the full training set.

\begin{figure}[!ht]
    \centering
    \captionsetup{font=scriptsize}
%\includegraphics[width=0.5\textwidth]{figures/IP_sub2.png}
\includegraphics[width=0.8\textwidth]{figures/sample_efficient.pdf}
\caption{Comparison to the SpectralFormer on subset of training samples with IP dataset. Our model learns better from limited number of examples.}
\label{fig:ip_sub}
\end{figure}

\subsection{Ablation Study}
\partitle{Attention order} To investigate the performance gain of the proposed model and to understand the effects of the spectral-spatial attention order, we  conduct comparison experiments by changing the multi-head attention order of spectral and spatial inside each transformer block. Table \ref{tab:attn_order} indicates that firstly performing spectral attention outperforms firstly performing spatial attention. [In detail, REASON?]
\begin{table}[!ht]
\centering
\captionsetup{font=scriptsize}
\scalebox{0.65}{
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Attention order}} & \multicolumn{3}{c|}{Indian Pines}                                                                      & \multicolumn{3}{c|}{Houston2013}                                                                       & \multicolumn{3}{c|}{Pavia University}                                                                  \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      \\ \hline
Spatial -\textgreater Spectral                         & \multicolumn{1}{l|}{87.44}          & \multicolumn{1}{l|}{92.25}          & \multicolumn{1}{l|}{0.856} & \multicolumn{1}{l|}{87.14}          & \multicolumn{1}{l|}{88.18}          & \multicolumn{1}{l|}{0.860} & \multicolumn{1}{l|}{85.60}          & \multicolumn{1}{l|}{91.29}          & \multicolumn{1}{l|}{0.814} \\ \hline
Spectral -\textgreater Spatial                         & \multicolumn{1}{c|}{\textbf{89.80}} & \multicolumn{1}{c|}{\textbf{94.69}} & \textbf{0.883}             & \multicolumn{1}{c|}{\textbf{88.49}} & \multicolumn{1}{c|}{\textbf{89.74}} & \textbf{0.875}             & \multicolumn{1}{c|}{\textbf{91.28}} & \multicolumn{1}{c|}{\textbf{92.25}} & \textbf{0.884}             \\ \hline
\end{tabular}
}
\caption{Does the order of spectral and spatial attention matter? Indeed, including spatial attention after spectral leads to higher improvement.}
\label{tab:attn_order}
\end{table}

\partitle{Positional embedding} In addition, we have also studied the positional embedding factor to the SpectralFormer and the proposed method. Table \ref{tab:position} represents the results, from which we can see that positional embedding improves the classification performance.
\begin{table}[!ht]
\centering
\captionsetup{font=scriptsize}
\scalebox{0.65}{
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}}                     & \multicolumn{3}{c|}{Indian Pines}                                                                      & \multicolumn{3}{c|}{Houston2013}                                                                       & \multicolumn{3}{c|}{Pavia University}                                                                  \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                           & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                      \\ \hline
SpectralFormer                                                   & \multicolumn{1}{c|}{\textbf{78.97}} & \multicolumn{1}{c|}{\textbf{85.39}} & \textbf{0.760}             & \multicolumn{1}{c|}{\textbf{85.08}} & \multicolumn{1}{c|}{\textbf{86.39}} & \textbf{0.838}             & \multicolumn{1}{c|}{\textbf{84.64}} & \multicolumn{1}{c|}{\textbf{86.75}} & \textbf{0.799}             \\ \hline
\begin{tabular}[c]{@{}l@{}}SpectralFormer\\  wo PE\end{tabular} & \multicolumn{1}{l|}{67.37}          & \multicolumn{1}{l|}{79.68}          & \multicolumn{1}{l|}{0.634} & \multicolumn{1}{l|}{82.45}          & \multicolumn{1}{l|}{82.62}          & \multicolumn{1}{l|}{0.810} & \multicolumn{1}{l|}{79.73}          & \multicolumn{1}{l|}{86.47}          & \multicolumn{1}{l|}{0.741} \\ \hline
Ours wo PE                                                      & \multicolumn{1}{l|}{79.63}          & \multicolumn{1}{l|}{85.35}          & \multicolumn{1}{l|}{0.768} & \multicolumn{1}{l|}{84.09}          & \multicolumn{1}{l|}{85.96}          & \multicolumn{1}{l|}{0.827} & \multicolumn{1}{l|}{84.69}          & \multicolumn{1}{l|}{87.18}          & \multicolumn{1}{l|}{0.794} \\ \hline
Ours                                                             & \multicolumn{1}{c|}{\textbf{89.80}} & \multicolumn{1}{c|}{\textbf{94.69}} & \textbf{0.883}             & \multicolumn{1}{c|}{\textbf{88.49}} & \multicolumn{1}{c|}{\textbf{89.74}} & \textbf{0.875}             & \multicolumn{1}{c|}{\textbf{91.28}} & \multicolumn{1}{c|}{\textbf{92.25}} & \textbf{0.884}             \\ \hline
\end{tabular}
}
\caption{Comparison of the SpectralFormer with or without positional embedding (PE), and the proposed method with or without PE.}
\label{tab:position}
\end{table}

% Structure of Attention 
\partitle{Pooling}
Due the speciality of HSIC, the global classification embedding can be pooled from either spectral wavebands dimension or spatial patch dimension. Pooling from spectral dimension aggregates information from each embedded spectral band of all patches, while pooling from spatial dimension aggregates information from each embedded patch of all spectral bands. Table \ref{tab:pooling} represents the experimental results, from which we can see that pooling from spatial patches performs better than pooling from spectral bands for all studied datasets. This indicates that the global features used for final classification benefit more from each patch embedding of all spectral bands.

\begin{table}[!ht]
\centering
\captionsetup{font=scriptsize}
\scalebox{0.65}{
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Pooling from}} & \multicolumn{3}{c|}{Indian Pines}                                                          & \multicolumn{3}{c|}{Houston2013}                                                           & \multicolumn{3}{c|}{Pavia University}                                                      \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                              & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          \\ \hline
Spectral bands                                      & \multicolumn{1}{c|}{83.54}          & \multicolumn{1}{c|}{92.61}              & {0.814}              & \multicolumn{1}{c|}{85.85}          & \multicolumn{1}{c|}{87.26}              & {0.846}              & \multicolumn{1}{c|}{91.05}          & \multicolumn{1}{c|}{92.16}              & {0.881}              \\ \hline
Spatial patches                                     & \multicolumn{1}{c|}{\textbf{89.80}} & \multicolumn{1}{c|}{\textbf{94.69}} & \textbf{0.883} & \multicolumn{1}{c|}{\textbf{88.49}} & \multicolumn{1}{c|}{\textbf{89.74}} & \textbf{0.875} & \multicolumn{1}{c|}{\textbf{91.28}} & \multicolumn{1}{c|}{\textbf{92.25}} & \textbf{0.884} \\ \hline
\end{tabular}
}
\caption{Comparison of pooling the global $class$ token from spectral dimension and from spatial dimension.}
\label{tab:pooling}
\end{table}

% Depth-Head


% Fusion
\partitle{Fusion} The spectral-spatial fusion can happen in early feature level, which is the proposed method, or in late class level. Different from feature level fusion network that contains spectral and spatial attention modules in the same transformer blocks, in the class level fusion network, spectral and spatial representations are extracted through two parallel transformer encoder branches separately. One branch consists of blocks that have spectral attention modules and feed-forward modules to extract spectral features, while the other branch consists of the same number of blocks that have spatial attention modules and feed-forward modules to extract spatial features. Finally, the extracted spectral and spatial features are added together as the input of the MLP head to make final classification. Table \ref{tab:fusion} shows the comparison results of these two fusion methods, which indicates that feature level spectral-spatial fusion outperforms class level fusion on all the studied datasets.

\begin{table}[!ht]
\centering
\captionsetup{font=scriptsize}
\scalebox{0.65}{
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Spectral-Spatial \\ Fusion\end{tabular}}} & \multicolumn{3}{c|}{Indian Pines}                                                          & \multicolumn{3}{c|}{Houston2013}                                                           & \multicolumn{3}{c|}{Pavia University}                                                      \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                                                                    & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa          \\ \hline
Class-level fusion                                                                                        & \multicolumn{1}{c|}{81.05}          & \multicolumn{1}{c|}{89.86}          & 0.786          & \multicolumn{1}{c|}{86.05}          & \multicolumn{1}{c|}{87.83}          & 0.848          & \multicolumn{1}{c|}{87.41}          & \multicolumn{1}{c|}{88.20}          & 0.833          \\ \hline
Feature-level fusion                                                                                      & \multicolumn{1}{c|}{\textbf{89.80}} & \multicolumn{1}{c|}{\textbf{94.69}} & \textbf{0.883} & \multicolumn{1}{c|}{\textbf{88.49}} & \multicolumn{1}{c|}{\textbf{89.74}} & \textbf{0.875} & \multicolumn{1}{c|}{\textbf{91.28}} & \multicolumn{1}{c|}{\textbf{92.25}} & \textbf{0.884} \\ \hline
\end{tabular}
}
\caption{Comparison of fusing spectral-spatial representations in class-level and feature-level.}
\label{tab:fusion}
\end{table}

\subsection{Further Analysis}
%\partitle{Attention analysis}
% Band attention analysis
% Class-level improvement analysis
\partitle{Class-level analysis} To investigate the performance gain of the proposed method in more detail, we compare the classification accuracy of each single class of Indian Pines dataset between our model and the SpectralFormer, and the results are visualized in Figure \ref{fig:ip_classes}. The categories are presented with the ascending order of the performance gap between our model and the SpectralFormer. As can be seen, except for the category of $corn$, of which the SpectralFormer gained $0.4\%$ higher OA than ours, our method performs equally or better than the SpectralFormer among all other classes. Particularly, in terms of detecting $woods$, $Soybean-clean$ and $Hay-windrowed$, our model reaches over $26\%$ accuracy than the SpectralFormer.

\begin{figure}[!ht]
    \centering
    \captionsetup{font=scriptsize}
\includegraphics[width=1.0\textwidth]{figures/IP_class.pdf}
\caption{Comparison to the SpectralFormer by each categories of IP dataset.}
\label{fig:ip_classes}
\end{figure}

\partitle{Alignment loss} To investigate the performance gain of applying global-local feature alignment loss in addition to cross-entropy loss function, we conduct the experiments to compare the SpectralFormer with and without alignment loss, and the proposed approach with and without alignment loss. Table \ref{tab:loss} lists the classification results, in which $\textbf{w AL}$ indicates with alignment loss and $\textbf{wo AL}$ denotes without alignment loss. It is clear that for both SpectralFormer and the proposed LAT-HISC networks, adding global-local feature alignment loss improves classification performance in a certain level.
\begin{table}[!ht]
\centering
\captionsetup{font=scriptsize}
\scalebox{0.65}{
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}}                   & \multicolumn{3}{c|}{Indian Pines}                                                                               & \multicolumn{3}{c|}{Houston2013}                                                                                & \multicolumn{3}{c|}{Pavia University}                                                                           \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                               & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                               & \multicolumn{1}{c|}{OA}             & \multicolumn{1}{c|}{AA}             & Kappa                               \\ \hline
SpectralFormer                                                 & \multicolumn{1}{c|}{78.97}          & \multicolumn{1}{c|}{85.39}          & 0.760                               & \multicolumn{1}{c|}{85.08}          & \multicolumn{1}{c|}{86.39}          & 0.838                               & \multicolumn{1}{c|}{84.64}          & \multicolumn{1}{c|}{86.75}          & 0.799                               \\ \hline
\begin{tabular}[c]{@{}l@{}}SpectralFormer\\  w AL\end{tabular} & \multicolumn{1}{l|}{\textbf{83.00}} & \multicolumn{1}{l|}{\textbf{89.40}} & \multicolumn{1}{l|}{\textbf{0.806}} & \multicolumn{1}{l|}{\textbf{87.13}} & \multicolumn{1}{l|}{\textbf{88.33}} & \multicolumn{1}{l|}{\textbf{0.860}} & \multicolumn{1}{l|}{\textbf{87.76}} & \multicolumn{1}{l|}{\textbf{91.72}} & \multicolumn{1}{l|}{\textbf{0.840}} \\ \hline
Ours wo AL                                                    & \multicolumn{1}{l|}{85.37}          & \multicolumn{1}{l|}{90.09}          & \multicolumn{1}{l|}{0.833}          & \multicolumn{1}{l|}{85.90}               & \multicolumn{1}{l|}{87.91}               & \multicolumn{1}{l|}{0.847}               & \multicolumn{1}{l|}{87.78}               & \multicolumn{1}{l|}{91.06}               & \multicolumn{1}{l|}{0.840}               \\ \hline
Ours                                                      & \multicolumn{1}{c|}{\textbf{89.80}} & \multicolumn{1}{c|}{\textbf{94.69}} & \textbf{0.883}                      & \multicolumn{1}{c|}{\textbf{88.49}} & \multicolumn{1}{c|}{\textbf{89.74}} & \textbf{0.875}                      & \multicolumn{1}{c|}{\textbf{91.28}} & \multicolumn{1}{c|}{\textbf{92.25}} & \textbf{0.884}                      \\ \hline
\end{tabular}
}
\caption{Comparison of the SpectralFormer with or without global-local feature alignment loss (AL), and the proposed approach with or without AL. }
\label{tab:loss}
\end{table}




\input{figures/table_ablation}
